FIG-OP: Exploring Large-Scale Unknown Environments on a Fixed Time Budget

We present a method for autonomous exploration of large-scale unknown environments under mission time constraints. We start by proposing the Frontloaded Information Gain Orienteering Problem (FIG-OP) -- a generalization of the traditional orienteering problem where the assumption of a reliable environmental model no longer holds. The FIG-OP addresses model uncertainty by frontloading expected information gain through the addition of a greedy incentive, effectively expediting the moment in which new area is uncovered. In order to reason across multi-kilometre environments, we solve FIG-OP over an information-efficient world representation, constructed through the aggregation of information from a topological and metric map. Our method was extensively tested and field-hardened across various complex environments, ranging from subway systems to mines. In comparative simulations, we observe that the FIG-OP solution exhibits improved coverage efficiency over solutions generated by greedy and traditional orienteering-based approaches (i.e. severe and minimal model uncertainty assumptions, respectively).

==> figures/old_Hierarchy_v3_figure.tex <==
% \phdone{Front Page Figure}
% \begin{figure}[t!]
% \centering
%     \begin{tikzpicture}
%     \node[anchor=south west,inner sep=0] (image) at (0,0) {\includegraphics[width=1\columnwidth]{figures/1_MultiFidelity.pdf}};
% 	    \begin{scope}[x={(image.south east)},y={(image.north west)}]
% 	    	%
% 	    	\node [font=\scriptsize,above left,align=right,black] at (1.03,0.66) {Frontier Map}; %
% 	    	\node [font=\scriptsize,above left,align=right,black] at (0.33,0.78) {Global IRM}; %
% 	    	\node [font=\scriptsize,above left,align=right,black] at (0.45,0.04) {Local Riskmap};
% 	    	\node [font=\scriptsize,above left,align=right,black] at (0.20,0.44) {\algname{} Path};
% 	    	\node [font=\scriptsize,above left,align=right,black] at (0.96,-0.02) {Robot};

% 	    \end{scope}
% 	\end{tikzpicture}	
%   \caption{Global Information RoadMap (IRM), Local Risk and Frontier Maps generated during Husky's autonomous exploration of the Limestone Mines of the Kentucky Underground, Nicholasville, KY.} \label{fig:hierarchy} 
% \end{figure}
